Redefining Normal: A Novel Object-Level Approach for Multi-Object Novelty Detection

In the realm of novelty detection, accurately identifying outliers in data without specific class information poses a significant challenge. While current methods excel in single-object scenarios, they struggle with multi-object situations due to their focus on individual objects. Our paper suggests a novel approach: redefining `normal' at the object level in training datasets. Rather than the usual image-level view, we consider the most dominant object in a dataset as the norm, offering a perspective that is more effective for real-world scenarios. Adapting to our object-level definition of `normal', we modify knowledge distillation frameworks, where a student network learns from a pre-trained teacher network. Our first contribution, DeFeND(Dense Feature Fine-tuning on Normal Data), integrates dense feature fine-tuning into the distillation process, allowing the teacher network to focus on object-level features with a self-supervised loss. The second is masked knowledge distillation, where the student network works with partially hidden inputs, honing its ability to deduce and generalize from incomplete data. This approach not only fares well in single-object novelty detection but also considerably surpasses existing methods in multi-object contexts. The implementation is available at: https://github.com/SMSD75/Redefining_Normal_ACCV24/tree/main

==> Figs/Rebuttal_Fig.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth, trim=4cm 5cm 2.5cm 2cm, clip]{Pictures/Fig_rebuttal_2.pdf}
    \captionsetup{skip=-5pt}
    \caption{\textbf{Object-centric biases in MNIST, CIFAR-10 and COCO.} COCO shows less bias and objects are not necessarily focused at the center.}
    \label{fig:rebuttal_fig}
\end{figure}
% \vspace{-10pt}

==> Tables/masking_ablations.tex <==
\begin{table*}[!htb]   
\setlength{\tabcolsep}{0.2em}
\aboverulesep = 0mm \belowrulesep = 0mm
\centering
\begin{tabular}{ccccccc}
\midrule
& Backbone & Num layer & Loss & Mask & \multicolumn{2}{c}{Results} \\
% \cline{8-9}
\cline{6-7}
          &      &    &   &            & CIFAR-10 & MVTecAD \\
\midrule
\multirow{3}{*}{With Masking}
& ViT-S16 & top5      & smooth $L_1$ & Random & 89.8 & 91.0 \\
& ViT-S16 & top5      & smooth $L_1$ & Guided & 90.0 & \textbf{91.4} \\
& ViT-S16 & top1      & $L_2$ & Guided & \textbf{93.4} & 88.1\\
\bottomrule
\multirow{2}{*}{Without Masking}
& ViT-S16 & top5      & smooth $L_1$ & - & 89.4 & 90.4 \\
& ViT-S16 & top1      & $L_2$ & - & 92.6 & 87.4\\
\bottomrule
\end{tabular}
\caption{\textbf{Masked MKD ablation studies.}\ya{split into multiple ablations for clarity}}
\label{table:masking_ablations}
\end{table*}


==> Tables/rebuttal_table.tex <==
\begin{table}[!t]
\centering
\aboverulesep = 0mm \belowrulesep = 0mm
\resizebox{\columnwidth}{!}{\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{\textbf{Uni-Class}} & & \multicolumn{2}{c}{\textbf{Multi-Class}} \\
\cline{2-4}
\cline{6-7}
& C10 & Pascal & COCO & & Pascal & COCO \\
% \midrule
% \midrule
DSVDD~[3] & 64.8 & 56.1 & 50.1 & & 47.3 & 49.4 \\
% \midrule
PatchCore~[2] & 67.2 & 68.3 & 62.1 & & 50.7 & 47.9 \\
RDAD~[1] & 86.5 & 58.6 & 47.9 & & 40.4 & 51.6 \\
% \midrule
KDAD~[4] & 87.2 & 82.8 & 75.4 & & 58.1 & 52.9 \\
\midrule
Ours & \textbf{98.6} & \textbf{95.4} & \textbf{94.5} & & \textbf{63.0} & \textbf{70.2} \\
% \midrule
% SimpleNet & - & - & & & \\
\bottomrule
\end{tabular}}

\caption{\textbf{Novelty detection results based on AUROC.} While some methods perform similarly on CIFAR-10 (RDAD vs. KDAD), their performance varies considerably on the proposed multi-object novelty detection setting. Our results are strong for all settings.}
\vspace{-1em}
\label{table:rebuttal_ablations}
\end{table}


